pFedUL: Layer-Aware Federated Unlearning for Personalized Federated Learning

Federated unlearning (FU) enables the removal of specific data contributions from federated learning (FL) models to comply with regulations such as the General Data Protection Regulation (GDPR). However, most existing FU methods are designed for the FedAvg paradigm, where all clients share a single global model. In practice, personalized federated learning (pFL) methods such as FedPer, FedRep, Ditto, and FedBN have become widely adopted due to their superior handling of non-IID data. These methods decompose the model into shared global layers and client-specific personalized layers, fundamentally altering the semantics of unlearning, yet this setting has received little attention. We formalize FU under the pFL paradigm, identifying a tension between unlearning completeness on shared layers and personalization preservation for remaining clients. We then propose pFedUL, a layer-aware selective unlearning framework comprising three components: (1) gradient-based layer-wise contribution attribution that separately quantifies the target client's influence on shared and personalized parameters, (2) adaptive selective unlearning that applies differentiated forgetting strategies across layer types, and (3) a lightweight recalibration protocol enabling remaining clients to restore personalization with minimal overhead. We further introduce two new metrics, Personalization Preservation Score (PPS) and Cross-client Fairness Index (CFI), to evaluate pFL-specific unlearning quality. Experiments on CIFAR-10, CIFAR-100, and FEMNIST under varying non-IID settings indicate that pFedUL achieves unlearning effectiveness comparable to full retraining while maintaining an average of 97.3\% personalized accuracy for remaining clients. Compared with six state-of-the-art FU methods adapted to the pFL setting, pFedUL consistently achieves superior personalization preservation.

==> Definitions/journalnames.tex <==
% Updated 05 January 2026 used for Y2026
%% --------------------------------------------------------------------
%\DeclareOption{}{%%
%		\gdef\@journal{}
%		\gdef\@journalfull{}
%		\gdef\@journalshort{}
%		\gdef\@doiabbr{}
%		\gdef\@ISSN{}
%		\gdef\@societyowner{}
%}
%% --------------------------------------------------------------------
%% Fields meanings:
%% - Option name: Journal website name (used in URL)
%% - @journal: Journal website name (used in URL)
%% - @journalshort: Short Name (ISO4)
%% - @journalfull: Journal full name
%% - @doiabbr: DOI abbreviation of the journal used in DOI numbers 10.32604/journalnameXXXX
%% - @ISSN: Journal E-ISSN number
%% - @continuouspages: use  for journals that use pagination
%% - @societyowner: Name of society owning the journal (for society journals)
%% --------------------------------------------------------------------
\DeclareOption{biocell}{%
	\gdef\@journal{biocell}
	\gdef\@journalshort{Biocell}
	\gdef\@journalfull{Biocell}
	\gdef\@doiabbr{biocell}
	\gdef\@ISSN{1667-5746}
	\gdef\@societyowner{}
}
\DeclareOption{chd}{%
	\gdef\@journal{chd}
	\gdef\@journalshort{Congenit Heart Dis}
	\gdef\@journalfull{Congenital Heart Disease}
	\gdef\@doiabbr{chd}
	\gdef\@ISSN{1747-0803}
	\gdef\@societyowner{}
}
\DeclareOption{cju}{%
	\gdef\@journal{cju}
	\gdef\@journalshort{Can J Urol}
	\gdef\@journalfull{Canadian Journal of Urology}
	\gdef\@doiabbr{cju}
	\gdef\@ISSN{1488-5581}
	\gdef\@societyowner{}
}
\DeclareOption{cl}{%
	\gdef\@journal{cl}
	\gdef\@journalshort{Chalcogenide Lett}
	\gdef\@journalfull{Chalcogenide Letters}
	\gdef\@doiabbr{cl}
	\gdef\@ISSN{1584-8663}
	\gdef\@societyowner{}
}
\DeclareOption{cmc}{%
 	\gdef\@journal{cmc}
	\gdef\@journalshort{Comput Mater Contin}
	\gdef\@journalfull{Computers, Materials \& Continua}
	\gdef\@doiabbr{cmc}
	\gdef\@ISSN{1546-2226}
	\gdef\@societyowner{}
}
\DeclareOption{cmes}{%
 	\gdef\@journal{cmes}
	\gdef\@journalshort{Comput Model Eng Sci}
	\gdef\@journalfull{Computer Modeling in Engineering \& Sciences}
	\gdef\@doiabbr{cmes}
	\gdef\@ISSN{1526-1506}
	\gdef\@societyowner{}
}
\DeclareOption{csse}{%
 	\gdef\@journal{csse}
	\gdef\@journalshort{Comput Syst Sci Eng}
	\gdef\@journalfull{Computer Systems Science and Engineering}
	\gdef\@doiabbr{csse}
	\gdef\@ISSN{0267-6192}
	\gdef\@societyowner{}
}% ISSN (print)
\DeclareOption{dedt}{%
 	\gdef\@journal{dedt}
	\gdef\@journalshort{Digit Eng Digit Twin}
	\gdef\@journalfull{Digital Engineering and Digital Twin}
	\gdef\@doiabbr{dedt}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}% No ISSN
\DeclareOption{ecn}{%
 	\gdef\@journal{ecn}
	\gdef\@journalshort{Eur Cytokine Netw}
	\gdef\@journalfull{European Cytokine Network}
	\gdef\@doiabbr{ecn}
	\gdef\@ISSN{1952-4005}
	\gdef\@societyowner{}
}
\DeclareOption{ee}{%
 	\gdef\@journal{ee}
	\gdef\@journalshort{Energy Eng}
	\gdef\@journalfull{Energy Engineering}
	\gdef\@doiabbr{ee}
	\gdef\@ISSN{1546-0118}
	\gdef\@societyowner{}
}
\DeclareOption{fdmp}{%
 	\gdef\@journal{fdmp}
	\gdef\@journalshort{Fluid Dyn Mater Process}
	\gdef\@journalfull{Fluid Dynamics \& Materials Processing}
	\gdef\@doiabbr{fdmp}
	\gdef\@ISSN{1555-2578}
	\gdef\@societyowner{}
}
\DeclareOption{fhmt}{%
 	\gdef\@journal{fhmt}
	\gdef\@journalshort{Front Heat Mass Transf}
	\gdef\@journalfull{Frontiers in Heat and Mass Transfer}
	\gdef\@doiabbr{fhmt}
	\gdef\@ISSN{2125-8629}
	\gdef\@societyowner{}
}% ISSN (print)
\DeclareOption{iasc}{%
 	\gdef\@journal{iasc}
	\gdef\@journalshort{Intell Autom Soft Comput}
	\gdef\@journalfull{Intelligent Automation \& Soft Computing}
	\gdef\@doiabbr{iasc}
	\gdef\@ISSN{2326-005X}
	\gdef\@societyowner{}
}
\DeclareOption{icces}{%
 	\gdef\@journal{icces}
	\gdef\@journalshort{Int Conf Comput Exp Eng Sci}
	\gdef\@journalfull{The International Conference on Computational \& Experimental Engineering and Sciences}
	\gdef\@doiabbr{icces}
	\gdef\@ISSN{1993-2815}
	\gdef\@societyowner{}
}
\DeclareOption{ijmhp}{%
 	\gdef\@journal{ijmhp}
	\gdef\@journalshort{Int J Ment Health Promot}
	\gdef\@journalfull{International Journal of Mental Health Promotion}
	\gdef\@doiabbr{ijmhp}
	\gdef\@ISSN{2049-8543}
	\gdef\@societyowner{}
}
\DeclareOption{jai}{%
 	\gdef\@journal{jai}
	\gdef\@journalshort{J Artif Intell}
	\gdef\@journalfull{Journal on Artificial Intelligence}
	\gdef\@doiabbr{jai}
	\gdef\@ISSN{2579-003X}
	\gdef\@societyowner{}
}
\DeclareOption{jbd}{%
 	\gdef\@journal{jbd}
	\gdef\@journalshort{J Big Data}
	\gdef\@journalfull{Journal on Big Data}
	\gdef\@doiabbr{jbd}
	\gdef\@ISSN{2579-0056}
	\gdef\@societyowner{}
}
\DeclareOption{jbic}{%
 	\gdef\@journal{jbic}
	\gdef\@journalshort{J Blockchain Intell Comput}
	\gdef\@journalfull{Journal of Blockchain and Intelligent Computing}
	\gdef\@doiabbr{jbic}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}% No ISSN
\DeclareOption{jcs}{%
 	\gdef\@journal{jcs}
	\gdef\@journalshort{J Cyber Secur}
	\gdef\@journalfull{Journal of Cyber Security}
	\gdef\@doiabbr{jcs}
	\gdef\@ISSN{2579-0064}
	\gdef\@societyowner{}
}
\DeclareOption{jihpp}{%
 	\gdef\@journal{jihpp}
	\gdef\@journalshort{J Inf Hiding Priv Prot}
	\gdef\@journalfull{Journal of Information Hiding and Privacy Protection}
	\gdef\@doiabbr{jihpp}
	\gdef\@ISSN{2637-4226}
	\gdef\@societyowner{}
}
\DeclareOption{jimh}{%
 	\gdef\@journal{jimh}
	\gdef\@journalshort{JIMH}
	\gdef\@journalfull{Journal of Intelligent Medicine and Healthcare}
	\gdef\@doiabbr{jimh}
	\gdef\@ISSN{2837-634X}
	\gdef\@societyowner{}
}
\DeclareOption{jiot}{%
 	\gdef\@journal{jiot}
	\gdef\@journalshort{J Internet Things}
	\gdef\@journalfull{Journal on Internet of Things}
	\gdef\@doiabbr{jiot}
	\gdef\@ISSN{2579-0080}
	\gdef\@societyowner{}
}
\DeclareOption{jnm}{%
 	\gdef\@journal{jnm}
	\gdef\@journalshort{J New Media}
	\gdef\@journalfull{Journal of New Media}
	\gdef\@doiabbr{jnm}
	\gdef\@ISSN{2579-0129}
	\gdef\@societyowner{}
}
\DeclareOption{jpa}{%
 	\gdef\@journal{jpa}
	\gdef\@journalshort{J Psychol Afr}
	\gdef\@journalfull{Journal of Psychology in Africa}
	\gdef\@doiabbr{jpa}
	\gdef\@ISSN{1815-5626}
	\gdef\@societyowner{}
}
\DeclareOption{jpm}{%
 	\gdef\@journal{jpm}
	\gdef\@journalshort{J Polym Mater}
	\gdef\@journalfull{Journal of Polymer Materials}
	\gdef\@doiabbr{jpm}
	\gdef\@ISSN{0976-3449}
	\gdef\@societyowner{}
}
\DeclareOption{jqc}{%
 	\gdef\@journal{jqc}
	\gdef\@journalshort{J Quantum Comput}
	\gdef\@journalfull{Journal of Quantum Computing}
	\gdef\@doiabbr{jqc}
	\gdef\@ISSN{2579-0145}
	\gdef\@societyowner{}
}
\DeclareOption{jrm}{%
 	\gdef\@journal{jrm}
	\gdef\@journalshort{J Renew Mater}
	\gdef\@journalfull{Journal of Renewable Materials}
	\gdef\@doiabbr{jrm}
	\gdef\@ISSN{2164-6341}
	\gdef\@societyowner{}
}
\DeclareOption{oncologie}{%
 	\gdef\@journal{oncologie}
	\gdef\@journalshort{Oncologie}
	\gdef\@journalfull{Oncologie}
	\gdef\@doiabbr{oncologie}
	\gdef\@ISSN{1765-2839}
	\gdef\@societyowner{}
}
\DeclareOption{or}{%
 	\gdef\@journal{or}
	\gdef\@journalshort{Oncol Res}
	\gdef\@journalfull{Oncology Research}
	\gdef\@doiabbr{or}
	\gdef\@ISSN{1555-3906}
	\gdef\@societyowner{}
}
\DeclareOption{phyton}{%
 	\gdef\@journal{phyton}
	\gdef\@journalshort{Phyton-Int J Exp Bot}
	\gdef\@journalfull{Phyton-International Journal of Experimental Botany}
	\gdef\@doiabbr{phyton}
	\gdef\@ISSN{1851-5657}
	\gdef\@societyowner{}
}
\DeclareOption{rig}{%
 	\gdef\@journal{rig}
	\gdef\@journalshort{Rev Int Géomatique}
	\gdef\@journalfull{Revue Internationale de Géomatique}
	\gdef\@doiabbr{rig}
	\gdef\@ISSN{2116-7060}
	\gdef\@societyowner{}
}
\DeclareOption{rimni}{%
 	\gdef\@journal{rimni}
	\gdef\@journalshort{Revista Internacional de Métodos Numéricos para Cálculo y Diseño en Ingeniería}
	\gdef\@journalfull{Rev Int méTodos Numér Cálc Diseño Ing}
	\gdef\@doiabbr{rimni}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{sdhm}{%
 	\gdef\@journal{sdhm}
	\gdef\@journalshort{Struct Durab Health Monit}
	\gdef\@journalfull{Structural Durability \& Health Monitoring}
	\gdef\@doiabbr{sdhm}
	\gdef\@ISSN{1930-2991}
	\gdef\@societyowner{}
}
\DeclareOption{zkg}{%
 	\gdef\@journal{zkg}
	\gdef\@journalshort{ZKG Int}
	\gdef\@journalfull{ZKG International}
	\gdef\@doiabbr{zkg}
	\gdef\@ISSN{2366-1313}
	\gdef\@societyowner{}
}
\DeclareOption{notspecified}{%
	\gdef\@journal{notspecified}
	\gdef\@journalfull{Journal Not Specified}
	\gdef\@journalshort{Journal Not Specified}
	\gdef\@doiabbr{journal}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
\DeclareOption{test}{%
	\gdef\@journal{test}
	\gdef\@journalfull{TEST}
	\gdef\@journalshort{TEST}
	\gdef\@doiabbr{test}
	\gdef\@ISSN{}
	\gdef\@societyowner{}
}
